Hyperbolic Representation Learning: Revisiting and Advancing

The non-Euclidean geometry of hyperbolic spaces has recently garnered considerable attention in the realm of representation learning. Current endeavors in hyperbolic representation largely presuppose that the underlying hierarchies can be automatically inferred and preserved through the adaptive optimization process. This assumption, however, is questionable and requires further validation. In this work, we first introduce a position-tracking mechanism to scrutinize existing prevalent \hlms, revealing that the learned representations are sub-optimal and unsatisfactory. To address this, we propose a simple yet effective method, hyperbolic informed embedding (HIE), by incorporating cost-free hierarchical information deduced from the hyperbolic distance of the node to origin (i.e., induced hyperbolic norm) to advance existing \hlms. The proposed method HIE is both task-agnostic and model-agnostic, enabling its seamless integration with a broad spectrum of models and tasks. Extensive experiments across various models and different tasks demonstrate the versatility and adaptability of the proposed method. Remarkably, our method achieves a remarkable improvement of up to 21.4\% compared to the competing baselines.

==> results/shallow_50__link_settings.tex <==
\begin{tabular}{@{}ccccc|ccc|ccc@{}}
\toprule
\multicolumn{2}{c|}{Links}                & \multicolumn{3}{c|}{75\%Training Links}               & \multicolumn{3}{c|}{50\%Training Links}               & \multicolumn{3}{c}{25\%Training Links}               \\ 
\multicolumn{2}{c|}{Dimension}                        & 8          & 64         & 256        & 8          & 64         & 256        & 8          & 64         & 256        \\ \midrule \midrule
\multirow{4}{*}{AUC} & \multicolumn{1}{c|}{Euclidean} & $61.1\pm2.4$ & $72.2\pm0.5$ & $73.5\pm0.4$ & $56.8\pm0.6$ & $61.9\pm0.5$ & $63.8\pm0.4$ & $53.5\pm0.2$ & $54.3\pm0.3$ & $54.1\pm0.2$ \\
                     & \multicolumn{1}{c|}{Hyperbolic}  & $65.2\pm3.2$ & $74.9\pm0.4$ & $77.0\pm0.3$ & $59.3\pm1.7$ & $67.8\pm0.5$ & $69.8\pm0.14$ & $52.9\pm0.5$ & $53.7\pm0.5$ & $55.0\pm0.4$ \\
                     & \multicolumn{1}{c|}{Ours}      & $\textbf{72.0}\pm0.9$ & $\textbf{80.7}\pm0.4$ & $\textbf{82.5}\pm0.2$ & $\textbf{66.6}\pm0.6$ & $\textbf{74.4}\pm0.3$ & $\textbf{76.4}\pm0.2$ & $\textbf{58.1}\pm1.1$ & $\textbf{63.9}\pm0.4$ & $\textbf{66.8}\pm0.4$ \\
                     & \multicolumn{1}{c|}{$\Delta$(\%)}          & $+10.4$      & $+7.7$       & $+7.1$       & $+12.3$      & $+9.7$       & $+9.6$       & $+8.6$       & $+17.7$      & $+21.4$      \\ \midrule
\multirow{4}{*}{AP}  & \multicolumn{1}{c|}{Euclidean} & $58.7\pm1.3$ & $69.7\pm0.5$ & $71.4\pm0.7$ & $55.2\pm0.6$ & $60.6\pm0.4$ & $61.6\pm0.5$ & $52.2\pm0.2$ & $52.8\pm0.6$ & $52.3\pm0.1$ \\
                     & \multicolumn{1}{c|}{Hyperbolic}  & $62.3\pm2.7$ & $71.3\pm0.7$ & $72.7\pm0.4$ & $57.0\pm1.4$ & $65.5\pm0.6$ & $67.3\pm0.2$ & $51.9\pm0.7$ & $52.4\pm0.8$ & $54.1\pm0.7$ \\
                     & \multicolumn{1}{c|}{Ours}      & $\textbf{66.6}\pm1.0$ & $\textbf{75.0}\pm0.4$ & $\textbf{76.4}\pm0.3$ & $\textbf{62.5}\pm0.7$ & $\textbf{70.00}\pm0.3$ & $\textbf{71.5}\pm0.2$ & $\textbf{56.1}\pm1.0$ & $\textbf{62.6}\pm0.6$ & $\textbf{65.2}\pm0.6$ \\
                     &  \multicolumn{1}{c|}{$\Delta$(\%)}                              & $+6.9$       & $+5.2$       & $+5.0$       & $+9.6$       & $+6.9$       & $+6.3$       & $+7.4$       & $+18.7$      & $+20.4$      \\ \bottomrule
\end{tabular}
